ELT: Elastic Looped Transformers for Visual Generation

We introduce Elastic Looped Transformers (ELT), a highly parameter-efficient class of visual generative models based on a recurrent transformer architecture. While conventional generative models rely on deep stacks of unique transformer layers, our approach employs iterative, weight-shared transformer blocks to drastically reduce parameter counts while maintaining high synthesis quality. To effectively train these models for image and video generation, we propose the idea of Intra-Loop Self Distillation (ILSD), where student configurations (intermediate loops) are distilled from the teacher configuration (maximum training loops) to ensure consistency across the model's depth in a single training step. Our framework yields a family of elastic models from a single training run, enabling Any-Time inference capability with dynamic trade-offs between computational cost and generation quality, with the same parameter count. ELT significantly shifts the efficiency frontier for visual synthesis. With $4\times$ reduction in parameter count under iso-inference-compute settings, ELT achieves a competitive FID of $2.0$ on class-conditional ImageNet $256 \times 256$ and FVD of $72.8$ on class-conditional UCF-101.

==> tables/dit_images.tex <==
\begin{figure}[ht]
    \centering
    \begin{tabular}{ccccc}
    L = 2 & L = 4 & L = 6 & L = 8 & L = 10
        \includegraphics[width=0.3\linewidth]{figures/dit_images/siamese_ilsd_2.png} & \includegraphics[width=0.3\linewidth]{figures/dit_images/siamese_ilsd_2.png} &
        \includegraphics[width=0.3\linewidth]{figures/dit_images/siamese_ilsd_2.png} &
        \includegraphics[width=0.3\linewidth]{figures/dit_images/siamese_ilsd_2.png} &
        \includegraphics[width=0.3\linewidth]{figures/dit_images/siamese_ilsd_2.png}\\
    \end{tabular}
    \caption{Simple 2x2 grid}
    \label{tab:dit_images}
\end{figure}

==> tables/imagnet_dit.tex <==
\begin{table}[hbt!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
    \toprule
    Model & FID $\downarrow$ & L (for inference) & \# params\\
    \midrule
    Baseline - 16 layers & 1 & - & 1.1B \\
    Baseline - 32 layers & 1 & - & 2.1B \\
    \midrule   
    Loop w/o SJO ($1N \times 16L$) & 1&1  &1 \\
    Loop w/o SJO ($1N \times 32L$)& 1&  1&1 \\
    Loop w/o SJO ($4N \times 8L$)& 1& 1 &1 \\
    Loop w/o SJO ($4N \times 8L$)& 1&  1&1 \\
    \midrule
    Ours ($1N \times 16L$)& 1&1  &1 \\
    Ours ($1N \times 32L$)&1 & 1 &1 \\
    Ours ($4N \times 4L$)& 1& 1 & 1\\
    Ours ($4N \times 8L$)& 1& 1 & 1\\
    \bottomrule
\end{tabular}
}
\vspace{1mm}
\caption{\small \textbf{ Class-conditional Image Generation} on ImageNet $256\times256$ using DiT.}
\label{tab:img_dit}
\end{table}

==> tables/k600.tex <==
% \begin{table}[h]{
%     \centering
    \resizebox{\textwidth}{!}
    {
    \begin{tabular}{lccccc}
        \toprule
        Method & FVD $\downarrow$ & IS $\uparrow$ & \# params & \# steps & \# GFlops\\
        \midrule
        CogVideo$^{\square}$~\citep{hong2022cogvideo} & 109.2 & - &9.4B & - & -\\
        CCVS$^{\square}$ ~\citep{le2021ccvs} & 55.0$\pm$\textcolor{gray}{1.0} & - & - & - & -\\
        Phenaki$^{\square}$ ~\citep{villegas2022phenaki} & 36.4 $\pm$ \textcolor{gray}{0.2} & - & 1.8B & 48 & -\\
        TrIVD-GAN-FP$^{\square}$ ~\citep{luc2020transformation} & 25.7 $\pm$ \textcolor{gray}{0.7} & 12.54 $\pm$ \textcolor{gray}{0.06} & - & 1 & - \\
        Transframer$^{\square}$ ~\citep{nash2022transframer} & 25.4 & - & 662M & - & -\\
        RaMViD$^{\square}$ ~\citep{hoppe2022diffusion} & 16.5 & - &308M & 500 & - \\
        Video Diffusion$^{\square}$~\citep{ho2022video} & 16.2 $\pm$ \textcolor{gray}{0.3} & 15.64 & 1.1B & 128 & -\\
        MaGNeTS$^{\square}$~\citep{goyal2025maskedgenerativenestedtransformers} &  10.8 $\pm$ \textcolor{gray}{0.1} &  16.25 $\pm$ \textcolor{gray}{0.02} & 306M & 12 & $\sim$1.2k \\ 
        \midrule
        MAGVIT-B$^{\square}$~\citep{yu2023magvit} & 24.5$ \pm$ \textcolor{gray}{0.9} & - & 87M & 12 & $\sim$1.3k\\
        
        MAGVIT-L~\citep{yu2023magvit} & 7.2 $\pm$ \textcolor{gray}{0.1} & 16.48 $\pm$ \textcolor{gray}{0.01} &306M &12 & $\sim$ 4.3k\\
        
        % \hdashline
        
        Ours ($6N \times 4L$) &  12.4 $\pm$ \textcolor{gray}{0.1} &   {abc} $\pm$ \textcolor{gray}{0.02} & \textbf{76M} & 12 & $\sim$4.3k \\ 
        \bottomrule
    \end{tabular}
    }
%     \caption{\small \textbf{Frame prediction} on K600. $^\square$ denotes values taken from papers. $g_{x}$ denotes use of guidance only for final $x$ steps.}
%     \label{tab:k600_quant}
%     \vspace{-2mm}
%     }
% \end{table}

==> tables/throughput.tex <==
\begin{table}[h]
\centering
% \renewcommand{\arraystretch}{1.1}
\caption{\small \textbf{Throughput gains for \ours}. We report throughput (images/sec) ratio (\ours\ /\ Baseline) on a Google Cloud TPU v6e~\citep{googleclouduv6e} with $1\times1$ topology and inference batch size of 8. \ours\ achieves a peak speedup of $\emph{3.5}\times$ for model scale H.}
\vspace{-3mm}
\resizebox{0.4\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\ours\ & $d_{model}$ & Throughput Ratio \\ 
\midrule
$6N \times 2L$ (B)  & 768  & 1.0 \\
$8N \times 3L$ (L)  & 1024 & 2.9 \\
$7N \times 4L$ (XL) & 1152 & 3.3 \\
$8N \times 4L$ (H)  & 1280 & 3.5 \\
% G  & 1536 & 1.1 \\
\bottomrule
\end{tabular}
}
% \vspace{1mm}

\label{tab:thru}
\end{table}
